Distilling Coarse-to-Fine Semantic Matching Knowledge for Weakly Supervised 3D Visual Grounding

3D visual grounding involves finding a target object in a 3D scene that corresponds to a given sentence query. Although many approaches have been proposed and achieved impressive performance, they all require dense object-sentence pair annotations in 3D point clouds, which are both time-consuming and expensive. To address the problem that fine-grained annotated data is difficult to obtain, we propose to leverage weakly supervised annotations to learn the 3D visual grounding model, i.e., only coarse scene-sentence correspondences are used to learn object-sentence links. To accomplish this, we design a novel semantic matching model that analyzes the semantic similarity between object proposals and sentences in a coarse-to-fine manner. Specifically, we first extract object proposals and coarsely select the top-K candidates based on feature and class similarity matrices. Next, we reconstruct the masked keywords of the sentence using each candidate one by one, and the reconstructed accuracy finely reflects the semantic similarity of each candidate to the query. Additionally, we distill the coarse-to-fine semantic matching knowledge into a typical two-stage 3D visual grounding model, which reduces inference costs and improves performance by taking full advantage of the well-studied structure of the existing architectures. We conduct extensive experiments on ScanRefer, Nr3D, and Sr3D, which demonstrate the effectiveness of our proposed method.

==> egpaper_final.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}

% % Include other packages here, before hyperref.

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[breaklinks=true,bookmarks=false]{hyperref}

% \iccvfinalcopy % *** Uncomment this line for the final submission

% \def\iccvPaperID{****} % *** Enter the ICCV Paper ID here
% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \ificcvfinal\pagestyle{empty}\fi

% \begin{document}

% %%%%%%%%% TITLE
% \title{\LaTeX\ Author Guidelines for ICCV Proceedings}

% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle
% % Remove page # from the first page of camera-ready.
% \ificcvfinal\thispagestyle{empty}\fi

% %%%%%%%%% ABSTRACT
% \begin{abstract}
%    The ABSTRACT is to be in fully-justified italicized text, at the top
%    of the left-hand column, below the author and affiliation
%    information. Use the word ``Abstract'' as the title, in 12-point
%    Times, boldface type, centered relative to the column, initially
%    capitalized. The abstract is to be in 10-point, single-spaced type.
%    Leave two blank lines after the Abstract, then begin the main text.
%    Look at previous ICCV abstracts to get a feel for style and length.
% \end{abstract}

% %%%%%%%%% BODY TEXT
% \section{Introduction}

% Please follow the steps outlined below when submitting your manuscript to
% the IEEE Computer Society Press.  This style guide now has several
% important modifications (for example, you are no longer warned against the
% use of sticky tape to attach your artwork to the paper), so all authors
% should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the ICCV 2023 web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section,
% must be no longer than eight pages in length. The references section
% will not be included in the page count, and there is no limit on the
% length of the references section. For example, a paper of eight pages
% with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for ICCV 2023.}

% Overlength papers will simply not be reviewed.  This includes papers
% where the margins and formatting are deemed to have been significantly
% altered from those laid down by this style guide.  Note that this
% \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for
% supervised revisions of manuscripts.  The reviewing process cannot determine
% the suitability of the paper for presentation in eight pages if it is
% reviewed in eleven.  

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the
% version submitted for review.  The ruler is provided in order that
% reviewers may comment on particular lines in the paper without
% circumlocution.  If you are preparing a document using a non-\LaTeX\
% document preparation system, please arrange for an equivalent ruler to
% appear on the final output pages.  The presence or absence of the ruler
% should not change the appearance of any other content on the page.  The
% camera-ready copy should not contain a ruler. (\LaTeX\ users may uncomment
% the \verb'\iccvfinalcopy' command in the document preamble.)  Reviewers:
% note that the ruler measurements do not align well with the lines in the paper
% --- this turns out to be very difficult to do well when the paper contains
% many figures and equations, and, when done, looks ugly.  Just use fractional
% references (e.g.\ this line is $095.5$), although in most cases one would
% expect that the approximate location will be adequate.

% \subsection{Mathematics}

% Please number all of your sections and displayed equations.  It is
% important for readers to be able to refer to any particular equation.  Just
% because you didn't refer to it in the text doesn't mean some future readers
% might not need to refer to it.  It is cumbersome to have to use
% circumlocutions like ``the equation second from the top of page 3 column
% 1''.  (Note that the ruler will not be present in the final copy, so is not
% an alternative to equation numbers).  All authors will benefit from reading
% Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind
% review.  Blind review does not mean that one must remove
% citations to one's own work --- in fact, it is often impossible to
% review a paper unless the previous citations are known and
% available.

% Blind review means that you do not use the words ``my'' or ``our''
% when citing previous work.  That is all.  (But see below for
% tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say
% that you are Lucy Smith; it says that you are building on her
% work.  If you are Smith and Jones, do not say ``as we show in
% [7]'', say ``as Smith and Jones show in [7]'' and at the end of the
% paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper, we present a performance analysis of our
%    previous paper [1] and show it to be inferior to all
%    previously known methods.  Why the previous paper was
%    accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}

% An example of an acceptable paper:

% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper, we present a performance analysis of the
%    paper of Smith \etal [1] and show it to be inferior to
%    all previously known methods.  Why the previous paper
%    was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo
%    filter, a fundamental contribution to human knowledge''.
%    Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time,
% which covers similar or overlapping material, you may need to refer to that
% submission in order to explain the differences, just as you would if you
% had previously published related work.  In such cases, include the
% anonymized parallel submission~\cite{Authors14} as additional material and
% cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
% Supplied as additional material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be
% found elsewhere, and refer them to a technical report.  For conference
% submissions, the paper must stand on its own, and not {\em require} the
% reviewer to go to a tech report for further details.  Thus, you may say in
% the body of the paper ``further details may be found
% in~\cite{Authors14b}''.  Then submit the tech report as additional material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem that you tested using a tool that
% is widely known to be restricted to a single institution.  For example,
% let's say it's 1969, you have solved a key problem on the Apollo lander,
% and you believe that the ICCV70 audience would like to hear about your
% solution.  The work is a development of your celebrated 1968 paper entitled
% ``Zero-g frobnication: How being the only people in the world with access to
% the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.  Don't write ``We show how to
% improve our previous work [Anonymous, 1968].  This time we tested the
% algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors. Instead,
% write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.  This
%    system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] didn't
%    handle case B properly.  Ours handles it by including
%    a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo
%    lunar lander, and went all the way to the moon, don't
%    you know.  It displayed the following behaviors
%    which shows how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific conventions,
% reads better than the first version and does not explicitly name you as
% the authors.  A reviewer might think it likely that the new paper was
% written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been
% contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report the results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% \end{center}
%    \caption{Example of a caption.  It is set in Roman so mathematics
%    (always set in Roman: $B \sin A = A \sin B$) may be included without an
%    ugly clash.}
% \label{fig:long}
% \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a
% sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
% \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'',
% shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
% However, use it only when there are three or more authors.  Thus, the
% following is correct: ``
%    Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
% because reference~\cite{Alpher03} has just two authors.  If you use the
% \verb'\etal' macro provided, then you need not worry about double periods
% when used at the end of a sentence as in Alpher \etal.

% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.

% \begin{figure*}
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \end{center}
%    \caption{Example of a short caption, which should be centered.}
% \label{fig:short}
% \end{figure*}

% %------------------------------------------------------------------------
% \section{Formatting your paper}

% All text must be in a two-column format. The total allowable width of the
% text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
% cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
% $\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
% first page) should begin 1.0 inch (2.54 cm) from the top edge of the
% page. The second and following pages should begin 1.0 inch (2.54 cm) from
% the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
% cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
% paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
% high.

% Page numbers should be included for review submissions but not for the 
% final paper. Review submissions papers should have page numbers in the 
% footer with numbers centered and .75 inches (1.905 cm) from the bottom 
% of the page and start on the first page with the number 1.

% Page numbers will be added by the publisher to all camera-ready papers 
% prior to including them in the proceedings and before submitting the 
% papers to IEEE Xplore. As such, your camera-ready submission should 
% not include any page numbers. Page numbers should automatically be 
% removed by uncommenting (if it's not already) the line
% \begin{verbatim}
% % \iccvfinalcopy
% \end{verbatim}
% near the beginning of the .tex file.

% %-------------------------------------------------------------------------
% \subsection{Type-style and fonts}

% Wherever Times is specified, Times Roman may also be used. If neither is
% available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
% the first page. The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
% adverbs; do not capitalize articles, coordinate conjunctions, or
% prepositions (unless the title begins with such a word). Leave two blank
% lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type. This information is to
% be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
% double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
% inch or 0.422 cm). Make sure your text is fully justified---that is,
% flush left and flush right. Please do not place any additional blank
% lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in
% Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centered.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-,
% second-, and third-order headings.

% FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
% should be Times 12-point boldface, initially capitalized, flush left,
% with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
% should be Times 11-point boldface, initially capitalized, flush left,
% with one blank line before, and one after. If you require a third-order
% heading (we discourage it), use 10-point Times, boldface, initially
% capitalized, flush left, preceded by one blank line, followed by a period
% and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote {This is what a footnote looks like.  It
% often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral
% observations in
% the text (within parentheses, if you prefer, as in this sentence).  If you
% wish to use a footnote, place it at the bottom of the column on the page on
% which it is referenced. Use Times 8-point type, single-spaced.

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times,
% single-spaced, at the end of your paper. When referenced in the text,
% enclose the citation number in square brackets, for
% example~\cite{Authors14}.  Where appropriate, include the name(s) of
% editors of referenced books.

% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline
% Method & Frobnability \\
% \hline\hline
% Theirs & Frumpy \\
% Yours & Frobbly \\
% Ours & Makes one's heart Frob\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Results.   Ours is better.}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.  Please ensure that any point you wish to
% make is resolvable in a printed copy of the paper.  Resize fonts in figures
% to match the font in the body text, and choose line widths that render
% effectively in print.  Many readers (and reviewers), even of an electronic
% copy, will choose to print your paper in order to read it.  You cannot
% insist that they do otherwise, and therefore must not assume that they can
% zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use
% \verb+\includegraphics+, and to specify the  figure width as a multiple of
% the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage[dvips]{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.eps}
% \end{verbatim}
% }

% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the ICCV 2023 web page for a discussion
% of the use of color in your document.

% %------------------------------------------------------------------------
% \section{Final copy}

% You must include your signed IEEE copyright release form when you submit
% your finished paper. We MUST have this form before your paper can be
% published in the proceedings.

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> experiment/main.tex <==

\input{tables/scanrefer}
\section{Experiments}
\label{sec:exp}

\subsection{Datasets}
\noindent \textbf{ScanRefer.} The ScanRefer~\cite{chen2020scanrefer} dataset contain 51,583 descriptions of 11,046 objects from 800 Scannet~\cite{dai2017scannet} scenes. On average, each scene has 64.48 sentences and 13.81 objects. The data can be divided into ``Unique" and ``Multiple", depending on whether there are multiple objects of the same category as the target in the scene.

\noindent \textbf{Nr3D/Sr3D.} The Nr3D/Sr3D dataset~\cite{achlioptas2020referit3d} is also based on the indoor 3D scene dataset ScanNet~\cite{dai2017scannet}. Nr3D contains 41,503 human utterances collected by ReferItGame, and Sr3D contains 83,572 sentences automatically generated based on a ``target-spatial relationship-anchor object" template. Similar to the definition of ``Unique" and ``Multiple" in ScanRefer, Nr3D/Sr3D can be split into ``easy" and ``hard" subsets. The ``view-dep." and ``view-indep." subsets depend on whether the description is related to the speaker's view. \footnote{In the Nr3D/Sr3D datasets, the supervised task involves selecting the correct matching 3D box from a set of given boxes, with the instance matching accuracy serving as the evaluation metric. However, in the weakly-supervised setting, we predict the boxes from scratch and assess the IoU metrics, which cannot be directly compared to the results of supervised methods.}

\subsection{Evaluation Metric.} To evaluate the performance of our method and baselines on these three datasets, we adopt the ``$R@n, IoU@m$" metric. Specifically, this metric represents the percentage of at least one of the top-$n$ predicted proposals having an IoU greater than $m$ when compared to the ground-truth target bounding box. In our setting, $n \in {1, 3}$ and $m \in {0.25, 0.5}$. 

\subsection{Implementation Details.} We consider the 3DVG pipeline as consisting of off-the-shelf modules. In our practice, we use the pretrained GroupFree model~\cite{liu2021group} as our 3D object detector and employ the same matching architecture as the supervised 3DJCG model~\cite{cai20223djcg}.
The input point number $N_\mathrm{p}$, the proposal number $M_\mathrm{p}$, and the candidate number $K$ are set to 50000, 256 and 8, respectively. 
% The dimension of all hidden layers is 288. 
% The learning rate is set to 1e-3 with cosine annealing strategy. We employ AdamW optimizer\cite{loshchilov2018fixing} with the weight decay of 5e-4. The hyper-parameters $\lambda_1$, $\lambda_2$ and $\lambda_3$ are set to 2, 2 and 1, respectively. 
\textit{More details can be found in the supplementary material.}


\subsection{Compared Methods}

\noindent \textbf{Random.} We randomly select a candidate from all the proposals as the predicted result.

\noindent \textbf{MIL-Margin.} The MIL-Margin method~\cite{faghri2017vse++} proposes a max margin loss to enforce the score between a sentence and a paired scene to be higher than non-paired scenes, and vice versa. 

\noindent \textbf{MIL-NCE.} The MIL-NCE method~\cite{gupta2020contrastive} maximizes the InfoNCE lower bound on mutual information between the sentence and proposals from the paired scene, compared to non-corresponding pairs of scenes and sentences.

\noindent \textbf{Upper Bound.} The quality of the bounding boxes generated by the 3D object detector determines the upper bound performance of our model. We consider the maximum IoU between all the $M_\mathrm{p}$ object proposals and the ground-truth bounding box as the upper bound.

\input{tables/referit}
\input{tables/sup}

\subsection{Quantitative Comparison}
The performance results of our methods and baselines on ScanRefer and Nr3D/Sr3D are reported in Table \ref{table:scanrefer} and Table \ref{table:referit}, respectively, with the best results highlighted in \textbf{bold}. The comparison to supervised methods is presented in Table \ref{table:sup}. Although the 3D object detector pre-trained on ScanNet implicitly utilizes ground truth boxes on ScanNet, the object-sentence annotations are still unseen, and pre-training on ScanNet is only used to obtain more accurate proposals. To fully avoid annotations in ScanNet, we also evaluate results using a detector pre-trained on SUN RGB-D~\cite{song2015sun}. Despite the degradation caused by out-of-domain data, our method still shows significant improvement over baselines. By analyzing the evaluation results, we can observe the following facts:
\begin{itemize}

\item Our method achieves significant improvements over the Random method on all datasets, indicating the effectiveness of the coarse-to-fine semantic matching model in analyzing the similarity between objects and sentences when true object-sentence pairs are unavailable.
\item The results show that our method outperforms widely used MIL-based weakly supervised methods by a large margin, and even approaches the upper bound in the "Unique" subset of ScanRefer. This suggests that our proposed model can deeply exploit the alignment relationship between 3D scenes and sentences and identify the most semantically relevant object proposals.
\item Our coarse-to-fine semantic matching model significantly improves performance in the challenging "Multiple" subset of ScanRefer and "Hard" subset of Nr3D/Sr3D, where there are multiple interfering objects with the same category as the target object. This problem requires a comprehensive understanding of the sentence to distinguish the described object, which our model handles efficiently with the keywords semantic reconstruction module.
\item The performance improvement with the SUN RGB-D pre-trained backbone is relatively small on Nr3D and Sr3D datasets, possibly because the target objects are inherently more challenging to detect, and the pre-trained detector performs poorly due to out-of-domain data. The low grounding upper bound and inaccurate proposals make the training phase unstable. Nevertheless, our method outperforms all baselines, and when the detector is more reliable, our semantic matching model shows much more significant advantages on Nr3D/Sr3D.

\end{itemize}

\subsection{Ablation Study}
To further assess the effectiveness of each component in our design, we conduct ablation studies on the ScanRefer dataset.

\input{tables/abalation}

\subsubsection{Effectiveness of Semantic Matching Model}
\noindent \textbf{Coarse-to-Fine Matching Scores.}
We aim to examine the effect of each module in the coarse-to-fine semantic matching model. $\mathcal{L}_{cls}$ and $\mathcal{L}_{match}$ denote whether to use class similarity and feature similarity for coarsely selecting the top-$K$ candidates, respectively. $\mathcal{L}_{recon}$ represents using the reconstruct module to finely generate distilled pseudo labels for the selected $K$ candidates. If $\mathcal{L}_{recon}$ is not used, all the selected $K$ candidates's rewards are set directly to 1. Table \ref{table:abalation} shows that using $\mathcal{L}_{cls}$ or $\mathcal{L}_{match}$ alone can effectively aid the model in learning object-sentence pairs from the caption-level annotations, while joint usage of $\mathcal{L}_{cls}$ and $\mathcal{L}_{match}$ leads to better performance. Furthermore, the last two rows suggest that the fine-grained semantic matching module can effectively and comprehensively analyze the semantic similarity between the selected $K$ candidates and the sentence query.

\input{tables/num_can}
\input{tables/distill}
\input{figures/quali}

\noindent \textbf{Number of Coarse-grain Candidate.} 
We analyze the performance for varying numbers of coarse-grained candidates, $K \in {4, 8, 16, 32}$. As shown in Table \ref{table:num_can}, we observe that selecting 8 candidates yields the best results for fine-grained semantic matching. We tentatively infer the reason is that too small $K$ leaves out the possible proposal that covers the target object, while too large $K$ leads to selecing many proposals that are not relevant to the description due to the numerous objects in a 3D scene.


\subsubsection{Effectiveness of Knowledge Distillation}
\label{exp:distill}

% \noindent \textbf{Performance and Efficiency.} 
To investigate the effect of the semantic distillation in terms of performance and efficiency, we construct the baseline without knowledge distillation that removes the distillation loss $\mathcal{L}_{distill}$ during training and directly uses the coarse-to-fine semantic matching model for inference. As shown in Table \ref{table:distill}, distilling the semantic matching knowledge into the matching module of a two-stage 3DVG model brings a significant performance improvement. The well-studied structure of the existing 3DVG model enhances the generalization ability of our method. As for the efficiency, we observe that the distilled matching module is 3$\times$ smaller and 4$\times$ faster than the coarse-to-fine semantic matching model, demonstrating that the distilling operation reduces inference costs significantly. Meanwhile, we try to distill the knowledge into the matching modules of different supervised methods (SAT~\cite{yang2021sat}, 3DVG-Transformer~\cite{zhao20213dvg}, and 3DJCG~\cite{cai20223djcg}), the results show that the distillation fits well to different architectures.

% \input{tables/reward}

% \noindent \textbf{Matching Score Function for Distilled Pseudo Labels.} We compare our matching score function defined in Eq.\ref{eq:distill} with some typical mapping functions (i.e., one-hot, multi-hot, linear) in Table \ref{table:reward}. Our matching score function is apparently superior to other mapping functions. The underlying reason is that our function effectively balances the weights of proposals with different reconstruction losses so that we can generate distilled pseudo labels with more meaningful distribution. With such pseudo labels, knowledge of the coarse-to-fine semantic matching model can be migrated sufficiently.

\subsection{Qualitative Comparison}
As depicted in Figure~\ref{fig:quali}, we visualize the predicted bounding boxes in the corresponding 3D scene, where the green box denotes that the method predicts the correct object (IoU $\geq 0.5$ with the true box), and the red box indicates a wrong prediction.

In case (a), the target object is a \textit{trash can}. MIL-based methods may be misled by the presence of another object (\textit{bathroom counter}) in the sentence. While our method can filter out the objects that do not belong to the target category, benefiting from the coarse-grained candidate selection module. In case (b), there are six \textit{desks} in the scene. The MIL-based methods fail to localize the correct object, even though they figure out the target object (category) is \textit{desk}. With the fine-grained semantic matching module, our methods can better differentiate among these six \textit{desks} and choose the one best-matched to the sentence (``brown'' and ``under two monitors''). In case (c), the scene contains 32 different \textit{chairs}. Unfortunately, both our method and MIL-based methods fail in this case. However, we consider our method's predicted result acceptable. Firstly, the sentence query's expressions, such as ``near the doors'' and ``near the center'', are ambiguous and cannot give a precise location of the target object. Secondly, our method's predicted \textit{chair} is also consistent with the sentence description and is close to the true \textit{chair}. \textit{More qualitative cases can be found in the supplementary material.}

==> figures/quali_1.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=1\textwidth]{figures/quali_1.png}
    \caption{Qualitative Comparison between MIL-based methods and Ours. }
    \label{fig:quali_1}
\end{figure*}
    

==> introduction/abstract.tex <==
\begin{abstract}
3D visual grounding involves finding a target object in a 3D scene that corresponds to a given sentence query. Although many approaches have been proposed and achieved impressive performance, they all require dense object-sentence pair annotations in 3D point clouds, which are both time-consuming and expensive to obtain. To address this, we propose a weakly-supervised 3D visual grounding task that uses only coarse scene-sentence correspondences to learn object-sentence links. To accomplish this task, we design a novel semantic matching model that analyzes the semantic similarity between object proposals and sentences in a coarse-to-fine manner. Specifically, we first extract object proposals and coarsely select the top-K candidates based on feature and class similarity matrices. Next, we reconstruct the masked keywords of the sentence using each candidate one by one, and the reconstructed accuracy finely reflects the semantic similarity of each candidate to the query. Additionally, we distill the coarse-to-fine semantic matching knowledge into a typical two-stage 3D visual grounding model, which reduces inference costs and improves performance by taking full advantage of the well-studied structure of the existing architectures. We conduct extensive experiments on ScanRefer, Nr3D, and Sr3D, which demonstrate the effectiveness of our proposed method. \footnote{Our codes are provided in the supplementary material.}
\end{abstract}

==> introduction/introduction.tex <==

\section{Introduction}
\label{sec:intro}
\emph{3D Visual grounding} (3DVG) refers to the process of localizing an object in a scene based on a natural language sentence. The 3DVG task has recently gained attention due to its numerous applications. Despite the significant progress made in this area \cite{cai20223djcg, chen2020scanrefer, yuan2021instancerefer, zhao20213dvg, huang2022multi, yang2021sat}, all these approaches require bounding box annotations for each sentence query, which are laborious and expensive to obtain. For example, it takes an average of 22.3 minutes to annotate a scene in the Scannet-v2 dataset \cite{dai2017scannet}. Thus, we focus on weakly supervised training for 3DVG, which only requires scene-sentence pairs for training. Scene-level labels are much easier to obtain as they only indicate the presence of an object in the 3D scene without providing specific localization information.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/illustration.png}
\caption{(a). 3D visual grounding aims to find the object-sentence pair from the whole scene. The fully supervised setting requires all the dense ground-truth object-sentence labels for training, while the weakly supervised method only needs the coarse scene-sentence annotations. (b). Coarse-to-Fine Semantic Matching Model (bottom) analyzes the matching score of each proposal to the sentence, and the semantic matching knowledge is distilled to the two-stage 3DVG architecture (upper).}
\label{fig:illustration}
\end{figure}

However, weakly supervised 3DVG poses two challenges. Firstly, a 3D point cloud can contain numerous objects of various categories, and a sentence query may contain multiple objects besides the target object to aid in localization. Without knowledge of the ground-truth object-sentence pair, it is difficult to learn to link the sentence to its corresponding object from the enormous number of possible object-sentence pairs. Secondly, the 3DVG task often involves multiple interfering objects in the scene with the same class as the target object, and the target object must be distinguished based on its object attributes and the relations between objects described in the given sentence. As illustrated in Figure \ref{fig:illustration} (a), there are two trash cans in the scene, and the described target object can only be identified by fully comprehending the language description.

To address both challenges simultaneously, we propose a coarse-to-fine semantic matching model to measure the similarity between object proposals and sentences. Specifically, our model generates object-sentence matching scores from scene-sentence annotation, guided by coarse-to-fine semantic similarity analysis. Firstly, we calculate the object category similarity and feature similarity between all the proposals and the sentence. Combining these two similarities, we roughly select $K$ proposals with the highest similarity to the sentence, which can effectively filter out the proposals that do not belong to the target category. Secondly, the selected candidates would be used to reconstruct the masked keywords of the sentence, which can help the model fully and deeply understand the whole sentence. Since the target object and the sentence query are semantically consistent, the more the candidate and the target object overlap, the more accurate its predicted keywords will be. The object-sentence matching score of each candidate can be measured by its reconstruction loss. Eventually, in order to reduce inference time and make full use of the structure of existing 3DVG models, we utilize knowledge distillation\cite{hinton2015distilling} to migrate the knowledge of the coarse-to-fine semantic matching model to a typical two-stage 3DVG model, where the distilled pseudo labels are generated by the object-sentence matching scores.

%To simultaneously address both challenges, we propose a coarse-to-fine semantic matching model that measures the similarity between object proposals and sentences. Our model generates object-sentence matching scores from scene-sentence annotations, guided by coarse-to-fine semantic similarity analysis. Firstly, we calculate the object category similarity and feature similarity between all the proposals and the sentence. By combining these two similarities, we roughly select $K$ proposals with the highest similarity to the sentence, effectively filtering out the proposals that do not belong to the target category. Secondly, the selected candidates are used to reconstruct the masked keywords of the sentence, aiding the model in fully and deeply understanding the whole sentence. Since the target object and the sentence query are semantically consistent, the more the candidate and the target object overlap, the more accurate the predicted keywords will be. The object-sentence matching score of each candidate is measured by its reconstruction loss. Finally, in order to reduce inference time and make full use of the structure of existing 3DVG models, we utilize knowledge distillation\cite{hinton2015distilling} to transfer the knowledge of the coarse-to-fine semantic matching model to a typical two-stage 3DVG model, where the distilled pseudo labels are generated by the object-sentence matching scores.

In summary, the key contribution of this paper is four-fold:
\begin{itemize}
    \item[$\bullet$] To the best of our knowledge, this paper is the first work to address weakly supervised 3DVG, which eliminates the need for expensive and time-consuming dense object-sentence annotations and instead requires only scene-sentence level labels.
    \item[$\bullet$] We approach weakly supervised 3DVG as a coarse-to-fine semantic matching problem and propose a coarse-to-fine semantic matching model to analyze the similarity between each proposal and the sentence.
    \item[$\bullet$] We distill the knowledge of the coarse-to-fine semantic matching model into a two-stage 3DVG model, which fully leverages the well-studied network structure design, leading to improved performance and reduced inference costs.
    \item[$\bullet$] Experiments conducted on three wide-used datasets ScanRefer~\cite{chen2020scanrefer}, Nr3D~\cite{achlioptas2020referit3d} and Sr3D~\cite{achlioptas2020referit3d} demonstrate the effectiveness of our method. 
\end{itemize}


==> method/architecture.tex <==
\subsection{Model Architecture}
As depicted in Figure \ref{fig:overall}, our model utilizes a two-stage grounding pipeline. In the first stage, we employ a pre-trained 3D object detector to extract $M_\mathrm{p}$ object proposals from the given point cloud. In the second stage, we propose a coarse-to-fine semantic matching process to evaluate the degree of matchness between each proposal and the sentence query. We generate a pseudo label based on this matching process, which is subsequently utilized to distill matching knowledge into an effective matching architecture. This significantly enhances the inference efficiency of the model.

% The 3DVG pipeline is constructed in a mainstream two-stage paradigm, $i.e.$, object detection and cross-modal matching. We use a pre-trained 3D object detector to extract $M_\mathrm{p}$ object proposals from the given point cloud. The textual and object features are generated from the textual and attribute encoder, respectively. Then, the predict module carries out the cross-modal matching between objects and the sentence query.

Specifically, the coarse-to-fine process comprises two steps. Firstly, we coarsely extract the top $K$ object proposals, which are referred to as candidates, by computing the object-sentence similarity matrix between all proposals and the sentence query. Secondly, we generate a more accurate pseudo label by considering the semantic reconstruction result of each candidate-sentence pair. Further details will be explained in Section~\ref{sec:method_coarse} and Section~\ref{sec:method_fine}.

% Finally, with the assist of the pseudo labels generated from the semantic matching model, we train the predict module in the manner of knowledge distillation, which will be discussed in Section~\ref{sec:method_distill}.

% we follow the mainstream methods in the field of 3D visual grounding to construct a two-stage paradigm, i.e., language-irrelevant detection and cross-modal matching.

% The detection stage contains a pretrained 3D object detector which detects all the possible objects in the given point cloud and an attribute encoding module which aggregates the attribute features into the initial object features.

% The matching stage is devised by a coarse-to-fine pseudo label generating strategy, which contains a coarse-grained candidate selection module and a fine-grained label generation module. The coarse label selection module first select top-K possible candidates with assist of the class similarity and the feature similarity between object proposals and the language query. Next, the fine label generation module produces a more accurate pseudo label according to the semantic reconstruction result of each candidate-query pair. Finally, the predict module can be trained with the generated pseudo labels.

==> method/coarse.tex <==
\subsection{Coarse-grained Candidate Selection}
\label{sec:method_coarse}
% \paragraph{Textual Encoder}
% We use the 300d GloVe word2vec embedding\cite{pennington2014glove} to extract textual features. Then we feed them into a GRU cell and get the output features \tilde{\mathbf{Q}}\in\mathbb{R}^{N_\mathrm{q}\times d}\tilde{\mathbf{Q}}\in\mathbb{R}^{N_\mathrm{q}\times d}. Moreover, a global textual feature \tilde{\mathbf{q}}\in\mathbb{R}^d\tilde{\mathbf{q}}\in\mathbb{R}^d is also generated from the GRU cell to predict the target class of each language query. The class prediction of language query is denoted as \mathbf{q}^{\mathrm{cls}}\in\mathbb{R}^{N_\mathrm{c}^{\mathrm{q}}}\mathbf{q}^{\mathrm{cls}}\in\mathbb{R}^{N_\mathrm{c}^{\mathrm{q}}}, where N_\mathrm{c}^\mathrm{q}N_\mathrm{c}^\mathrm{q} is the number of target classes.
\paragraph{Object-Sentence Similarity.}
Although we have extracted numerous high-quality object proposals from the pre-trained 3D object detector, identifying the best-matched proposal with the sentence query is still challenging. This is because a 3D scene may contain many different classes of objects, and the semantic spaces between objects and the sentence are not aligned. To overcome this challenge, we propose calculating a similarity matrix between the objects and the sentence query based on both class and feature levels.

% Following the most implementations of 3DVG models, we obtain the class predictions of the objects and the query by the predict heads simply added after the object detector and the textual encoder, respectively (the object's predict head is pre-trained while the query's one is not). 
For the class level, we can obtain the object class from the pre-trained 3D object detector and the text class from a text classifier. For simplicity, we choose to train the text classifier from scratch and the classification loss $\mathcal{L}_{cls}$ is a simple cross-entropy loss. Considering that the object detector might be pre-trained on another dataset, the object class set and the text class set may be inconsistent. Therefore, before directly comparing the object proposals and the sentence, we need to transfer the object class prediction to the target text class. To achieve this, we propose using a class transform matrix  $\mathbf{M}^\mathrm{c}\in\mathbb{R}^{N_\mathrm{o}^\mathrm{c}\times N_\mathrm{q}^\mathrm{c}}$ for class alignment. The matrix is based on the cosine similarity between the GloVe embeddings of different class names. Here, $N_\mathrm{o}^\mathrm{c}$ and $N_\mathrm{q}^\mathrm{c}$ denote the number of object classes and the number of words in the sentence query, respectively.

For the feature level, we align the feature representations of the objects and the sentence query using a contrastive learning approach. Specifically, we pull the positive object-query pairs in the same scene closer and push the negative pairs further apart in the semantic space. To achieve this, all the object-query pairs in the same scene are considered as positive pairs $\mathbb{P}$, while those from different scenes are considered as negative pairs $\mathbb{N}$. The feature matching loss for object-sentence feature alignment can be computed by

% \begin{scriptsize}
\begin{equation}
\mathcal{L}_{match}=-\operatorname{log}\left(\frac{\sum\limits_{(\mathbf{p}, \mathbf{q})\in\mathbb{P}}e^{\phi(\mathbf{p},\mathbf{q})}}{\sum\limits_{(\mathbf{p}, \mathbf{q})\in\mathbb{P}}e^{\phi(\mathbf{p},\mathbf{q})}+
\sum\limits_{(\mathbf{p}^{'}, 
\mathbf{q})\in\mathbb{N}}e^{\phi(\mathbf{p}^{'},\mathbf{q})}}\right),
\end{equation}
% \end{scriptsize}

\noindent
where $\mathbf{p}$ represents an object proposal and $\mathbf{q}$ a sentence query. $B$ is the batch size. $\phi$ is the feature similarity function, which is a dot product in our practice.

We get the object-sentence similarity $\mathbf{\hat{s}}\in\mathbb{R}^{M_\mathrm{p}}$ by
\begin{equation}
\mathbf{\hat{s}}=\phi(\mathbf{\tilde{P}}^{\mathrm{c}}\mathbf{M}^\mathrm{c},\mathbf{\tilde{Q}}^\mathrm{c})+\phi(\mathbf{\tilde{P}},\mathbf{\tilde{Q}}),
\end{equation}
where $\mathbf{\tilde{P}}\in\mathbb{R}^{M_\mathrm{p}\times d}$ / $\mathbf{\tilde{Q}}\in\mathbb{R}^{N_\mathrm{q}\times d}$ is the encoded object/sentence feature, and $\mathbf{\tilde{P}}^{\mathrm{c}}\in\mathbb{R}^{N_\mathrm{o}^\mathrm{c}}$ / $\mathbf{\tilde{Q}}^\mathrm{c}\in\mathbb{R}^{N_\mathrm{q}^\mathrm{c}}$ is the object/sentence class prediction. $\phi$ is a similarity function ($e.g.$, cosine similarity or dot product). $M_\mathrm{p}$ is the number of object proposals. $d$ is the hidden dimension.


% We denote the extracted object proposals as 


% Considering that the object detector we use may be pretrained on another dataset, whose class collection is not consist to that of the current dataset, we construct a class transform matrix \mathbf{M}^\mathrm{cls}\in\mathbb{R}^{N_\mathrm{c}^{obj}\times N_\mathrm{c}^{q}}\mathbf{M}^\mathrm{cls}\in\mathbb{R}^{N_\mathrm{c}^{obj}\times N_\mathrm{c}^{q}} based on the cosine similarity between the GloVe embeddings of different class labels. Now the transformed object class prediction \hat{\mathbf{D}}^\mathrm{obj}=\mathbf{D}^\mathrm{obj}\cdot\mathbf{M}^\mathrm{cls}\in\mathbb{R}^{M_\mathrm{p}\times N_\mathrm{c}^\mathrm{q}}\hat{\mathbf{D}}^\mathrm{obj}=\mathbf{D}^\mathrm{obj}\cdot\mathbf{M}^\mathrm{cls}\in\mathbb{R}^{M_\mathrm{p}\times N_\mathrm{c}^\mathrm{q}} is aligned to the query class prediction \mathbf{q}^{\mathrm{cls}}\mathbf{q}^{\mathrm{cls}}. Then we calculate the object-query class similarity \mathbf{s}^\mathrm{c}=\{s_i^\mathrm{c}\}_{i=1}^{M_\mathrm{p}}\in\mathbb{R}^{M_\mathrm{p}}\mathbf{s}^\mathrm{c}=\{s_i^\mathrm{c}\}_{i=1}^{M_\mathrm{p}}\in\mathbb{R}^{M_\mathrm{p}}, where s_i^\mathrm{c}s_i^\mathrm{c} is the cosine similarity between \hat{\mathbf{D}}^\mathrm{obj}_i and  and \mathbf{q}^{\mathrm{cls}}\hat{\mathbf{D}}^\mathrm{obj}_i and  and \mathbf{q}^{\mathrm{cls}}.

% \paragraph{Multi-Instance Learning}
% Following some previous methods on weakly supervised vision-language tasks (cite), we use MIL-NCE\cite{miech2020end} to learn better feature representations for object proposals. We take all the object proposals and the corresponding language query as positive object-query pairs \mathbb{P}\mathbb{P}, and sample the objects and the queries from different 3D scene as negative pairs \mathbb{N}\mathbb{N}. The MIL-NCE objective can be formulated as:
% \begin{equation}
% \mathop{max}_{\operatorname{f},\operatorname{g}}\sum_{i=1}^{B}\mathop{log}\left(\frac{\sum\limits_{(\mathbf{x}, \mathbf{y})\in\mathbb{P}_i}e^{\operatorname{f}(\mathbf{x})^\top\operatorname{g}(\mathbf{y})}}{\sum\limits_{(\mathbf{x}, \mathbf{y})\in\mathbb{P}_i}e^{\operatorname{f}(\mathbf{x})^\top\operatorname{g}(\mathbf{y})}+\sum\limits_{(\mathbf{x}^{'}, \mathbf{y}^{'})\in\mathbb{N}_i}e^{\operatorname{f}(\mathbf{x}^{'})^\top\operatorname{g}(\mathbf{y}^{'})}}\right)
% \end{equation}where \mathbf{x}\mathbf{x} represents an object proposal and \mathbf{y}\mathbf{y} a language query. \operatorname{f}\operatorname{f} and \operatorname{g}\operatorname{g} are the object encoding function and the textual encoding function, respectively. We can simply calculate the object-query feature similarity \mathbf{s}^\mathrm{f}\in\mathbb{R}^{M_\mathrm{p}}\mathbf{s}^\mathrm{f}\in\mathbb{R}^{M_\mathrm{p}} by dot product between object features \tilde{\mathbf{C}}\tilde{\mathbf{C}} and the global textual feature \tilde{\mathbf{q}}\tilde{\mathbf{q}}.

\paragraph{Top-K Selection.}
According to the object-sentence similarity, we coarsely select the top $K$ candidates $\mathbf{\tilde{C}}\in\mathbb{R}^{K\times d}$ out of the $M_\mathrm{p}$ proposals $\mathbf{\tilde{P}}\in\mathbb{R}^{M_\mathrm{p}\times d}$, which can effectively filter out the proposals that do not belong to the target category.

% It would be ideal if we could directly choose the most similar object-sentence pair as the answer according to the object-sentence similarity. However, we cannot leave out the considerable noise brought by the process of the class prediction transform and the object-sentence feature alignment. To make better use of the information learned by object-sentence similarity, we coarsely select the top $K$ candidates $\mathbf{\tilde{C}}\in\mathbb{R}^{K\times d}$ out of the $M_\mathrm{p}$ proposals $\mathbf{\tilde{P}}\in\mathbb{R}^{M_\mathrm{p}\times d}$, which are supposed to be highly related to the sentence query due to their similar class predictions and feature representations. Then, we hope to get a deeper understanding of these $K$ candidates by a fine-grained semantic matching method.

% Next, we coarsely select top-K candidates, ranking them by the object-query similarity. These KK candidates are supposed to be in the same/similar class as that of the query target and also have similar semantic representations with the language query in the feature level. Thus, they are more likely to contain the best-matched object with the language query. Meanwhile, the process of top-K selection can effectively reduce the computation costs in the subsequent fine-grained module.


==> method/detection.tex <==
\subsection{Detection Stage}
\paragraph{3D Object Detector}
We use the pretrained GroupFree\cite{liu2021group} as our detection module. It takes the point cloud $P\in\mathbb{R}^{N_\mathrm{p}\times 3}$ as input and generates $M_\mathrm{p}$ possible proposals, where $M_\mathrm{p}$ is the upper bound number of the proposals. The output contains a set of point clusters $\mathbf{C}\in\mathbb{R}^{M_\mathrm{p}\times d}$, the axis-aligned bounding boxes $\mathbf{D}^\mathrm{bbox}\in\mathbb{R}^{M_\mathrm{p}\times 6}$, the objectness mask $\mathbf{D}^\mathrm{obj}\in\mathbb{R}^{M_\mathrm{p}\times 1}$ and the semantic class predictions $\mathbf{D}^\mathrm{cls}\in\mathbb{R}^{M_\mathrm{p}\times N_\mathrm{c}^\mathrm{obj}}$, where $d$ is the hidden dimension and $N_\mathrm{c}^\mathrm{obj}$ is the number of object classes. The point clusters $\mathbf{C}$ represents all object proposals with enriched point features. Each of the bounding box $\mathbf{D}^\mathrm{bbox}_{i}=(c_\mathrm{x}, c_\mathrm{y}, c_\mathrm{z}, s_\mathrm{x}, s_\mathrm{y}, s_\mathrm{z})$ consists of the box center $\mathbf{c}$ and the box size $\mathbf{s}$. 


\paragraph{Attribute Encoding Module}
To be consistent with the previous method\cite{cai20223djcg} in 3D VG task, we use an attribute encoding module to aggregate the initial object feature $\mathbf{C}$ with the attribute feature $\mathbf{A}=\{(\mathbf{a}^{\mathrm{obj}}_i, \mathbf{a}^{\mathrm{mul}}_i)\}_{i=1}^{M_\mathrm{p}}\in\mathbb{R}^{M_\mathrm{p}\times 155}$, where $\mathbf{a}^{\mathrm{obj}}_i\in\mathbb{R}^{27}$ is box center and corner coordinates, and $\mathbf{a}^{\mathrm{mul}}_i\in\mathbb{R}^{128}$ is multi-view RGB features that potentially contain the attribute information such as colors and materials. The attribute feature $\mathbf{A}$ is firstly encoded into the same dimension as the initial object features by a fully-connected layer. Then the encoded feature $\tilde{\mathbf{A}}\in\mathbb{R}^{M_\mathrm{p}\times d}$ can be added to the initial object feature to enhance it with more attribute information. After addition, we feed them to a multi-head self-attention layer\cite{vaswani2017attention} to further learn the mutual information between proposals. The output of the attribute encoding module is denoted as $\tilde{\mathbf{C}}\in\mathbb{R}^{M_\mathrm{p}\times d}$.

==> method/distill.tex <==
\subsection{Knowledge Distillation}
\label{sec:method_distill}
As mentioned earlier, a lower reconstruction loss indicates that the object candidate provides more consistent semantic information. A direct approach for object prediction is to select the candidate with the lowest reconstruction loss, as it is likely to be the best match. However, this coarse-to-fine matching process can be computationally expensive during inference. To address this issue, we distilled the semantic matching knowledge into a supervised 3DVG pipeline. This approach reduces the inference cost and leverages the existing powerful 3DVG architecture

For candidates, we calculate the reward according to their rank of $\mathcal{L}_{recon}^k$. The reward is reduced from one to zero, under the assumption that lower reconstruction loss gets better reward. The distilled pseudo labels $\mathbf{d}\in\mathbb{R}^{M_\mathrm{p}}$ can be generated by filling the rewards of candidates to their original indices and padding the non-candidate indices with zeros, following by a SoftMax operation. After all, we distill the knowledge by aligning the predict scores $\mathbf{s}\in\mathbb{R}^{M_\mathrm{p}}$ to the pseudo labels, where the predict scores are obtained from the powerful matching architecture. The distillation loss is:
\begin{equation}
\mathcal{L}_{distill}=-\sum_{i=1}^{M_\mathrm{p}}d_i\operatorname{log}(\frac{\operatorname{exp}(s_i)}{\sum_{j=1}^{M_\mathrm{p}}\operatorname{exp}(s_j)}).
\end{equation}

==> method/fine.tex <==
\subsection{Fine-grained Semantic Matching}
\label{sec:method_fine}
Given the $K$ object candidates, we propose a semantic reconstruction module to measure fine-grained semantic similarity between the objects and the sentence query.

As depicted in Figure~\ref{fig:overall}, we mask important words in the sentence query, such as the target object (\textit{table}), its attribute (\textit{blue}), and its relation to other objects (\textit{in front of}) in the scene. We reconstruct the masked words with the assistance of each candidate, respectively. The candidate that provides the most useful semantic information to predict the keywords and contains the least amount of noise is expected to be the best match.

We encode the masked sentence query using a textual encoder, denoted as $\tilde{\mathbf{Q}}^\mathrm{m}\in\mathbb{R}^{N_\mathrm{q}\times d}$. For the $k$-th candidate $\tilde{\mathbf{c}}^k\in\mathbb{R}^{d}$, we obtain the cross-modal semantic representation $\mathbf{f}^k=\{\mathbf{f}_i^k\}_{i=1}^{N_\mathrm{q}}\in\mathbb{R}^{N_\mathrm{q}\times d}$ using a transformer decoder, given by
\begin{equation}
    \mathbf{f}^k=\operatorname{Dec}(\tilde{\mathbf{Q}}^\mathrm{m},\tilde{\mathbf{c}}^k).
\end{equation}
To predict the masked words, we compute the energy distribution $\mathbf{e}^k=\{\mathbf{e}_i^k\}_{i=1}^{N_\mathrm{q}}\in\mathbb{R}^{N_\mathrm{q}\times d}$ over the vocabulary by
\begin{equation}
    \mathbf{e}_i^k=\mathbf{W}\mathbf{f}_i^k+\mathbf{b},
\end{equation}
where $\mathbf{e}_i^k\in\mathbb{R}^{N_\mathrm{v}}$ represents the energy distribution of the $i$-th predicted word, and $N_\mathrm{v}$ is the number of words in the vocabulary. $\mathbf{W}\in\mathbb{R}^{N_\mathrm{v}\times d}$ and $\mathbf{b}\in\mathbb{R}^{N_\mathrm{v}}$ are learnable parameters of a fully-connected layer.

Then, we adopt a reconstruction loss to train the semantic reconstruction module and make it effectively learn the key information from the object context to predict the masked words. Formally, we compute the sum of the negative log-likelihood of each masked word by
We use a reconstruction loss to train the semantic reconstruction module to effectively learn key information from the object context and predict the masked words. Specifically, we compute the negative log-likelihood of each masked word and sum them up by
\begin{equation}
\begin{aligned}
\mathcal{L}_{recon}^k&=-\sum_{i=1}^{N_\mathrm{q}-1}\operatorname{log}p(\mathbf{q}_{i+1}|\tilde{\mathbf{q}}_{1:i},\tilde{\mathbf{c}}^k)\\
&=-\sum_{i=1}^{N_\mathrm{q}-1}\operatorname{log}p(\mathbf{q}_{i+1}|\mathbf{e}_i^k),
\end{aligned}
\end{equation}
where $\mathcal{L}_{recon}^k$ is the reconstruction loss for the $k$-th candidate $\tilde{\mathbf{c}}^k$. Then the total loss for all the $K$ candidates is $\mathcal{L}_{recon}=\sum_{k=1}^K\mathcal{L}_{recon}^k$.

==> method/formulation.tex <==
\subsection{Problem Formulation}
In this paper, we address the task of weakly-supervised 3DVG. The input point cloud $\mathbf{P}=\{\mathbf{p}_i\}_{i=1}^{N_\mathrm{p}}$ contains point coordinates in 3D space, represented by $\mathbf{p}_i\in\mathbb{R}^{3}$. Correspondingly, a sentence query $\mathbf{Q}=\{\mathbf{q}_i\}_{i=1}^{N\mathrm{q}}$ is given to describe the object of interest. The objective of our model is to predict a 3D bounding box $\mathbf{B}=(\mathbf{c},\mathbf{r})$ that encompasses the object, where $\mathbf{c}=(c_x,c_y,c_z)$ represents the center of the box, and $\mathbf{r}=(r_x,r_y,r_z)$ represents the dimensions of the box. The number of input points and sentence length are denoted by $N_\mathrm{p}$ and $N_\mathrm{q}$, respectively. In the weakly-supervised setting, there are no bounding box annotations available during training.

==> method/main.tex <==
\section{Method}
\label{sec:method}

\input{figures/overall}

\input{method/formulation}

\input{method/architecture}

% \input{method/detection}

\input{method/coarse}

\input{method/fine}

\input{method/distill}

\input{method/train}

==> method/train.tex <==
\subsection{Training and Inference}
\label{sec:model_train}
% We train the model end-to-end via a multi-task loss function, containing classification loss $\mathcal{L}_{cls}$ of text classifier, feature matching loss $\mathcal{L}_{match}$ for object-sentence feature alignment, reconstruction loss $\mathcal{L}_{recon}$ of semantic reconstruction module, and distillation loss $\mathcal{L}_{distill}$ for knowledge distillation.

% \paragraph{Text Classification Loss.}
% The object class can be directly obtained from the pre-trained 3D object detector, while the text class prediction $\mathbf{q}^{\mathrm{cls}}\in\mathbb{R}^{N_\mathrm{q}^{\mathrm{cls}}}$ from the text classifier needs to be trained from scratch, where $N_\mathrm{q}^\mathrm{cls}$ is the number of different classes. The classification loss $\mathcal{L}_{cls}$ is a simple cross-entropy loss.

% \paragraph{Feature Matching Loss.}
% We take all the object proposals and the corresponding sentence query as positive object-sentence pairs $\mathbb{P}$, and sample the objects and the sentences from different 3D scenes as negative pairs $\mathbb{N}$. The feature matching loss for object-sentence feature alignment can be computed by

% \begin{scriptsize}
% \begin{equation}
% \mathcal{L}_{match}=-\sum_{i=1}^{B}\operatorname{log}\left(\frac{\sum\limits_{(\mathbf{p}, \mathbf{q})\in\mathbb{P}_i}\operatorname{exp}({\phi(\mathbf{p},\mathbf{q}))}}{\sum\limits_{(\mathbf{p}, \mathbf{q})\in\mathbb{P}_i}\operatorname{exp}({\phi(\mathbf{p},\mathbf{q})})+
% \sum\limits_{(\mathbf{p}^{'}, 
% \mathbf{q}^{'})\in\mathbb{N}_i}\operatorname{exp}({\phi(\mathbf{p}^{'},\mathbf{q}^{'}))}}\right)
% \end{equation}
% \end{scriptsize}

% \noindent
% where $\mathbf{p}$ represents an object proposal and $\mathbf{q}$ a sentence query. $B$ is the batch size. $\phi$ is the feature similarity function, which is a dot product in our practice.

% \paragraph{Reconstruction Loss.}
% Then, we adopt a reconstruction loss to train the semantic reconstruction module and make it effectively learn the key information from the object context to predict the masked words. Formally, we compute the sum of the negative log-likelihood of each masked word by
% We use a reconstruction loss to train the semantic reconstruction module to effectively learn key information from the object context and predict the masked words. Specifically, we compute the negative log-likelihood of each masked word and sum them up by
% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{recon}^k&=-\sum_{i=1}^{N_\mathrm{q}-1}\operatorname{log}p(\mathbf{q}_{i+1}|\tilde{\mathbf{q}}_{1:i},\tilde{\mathbf{c}}^k)\\
% &=-\sum_{i=1}^{N_\mathrm{q}-1}\operatorname{log}p(\mathbf{q}_{i+1}|\mathbf{e}_i^k),
% \end{aligned}
% \end{equation}
% where $\mathcal{L}_{recon}^k$ is the reconstruction loss for the $k$-th candidate $\tilde{\mathbf{c}}^k$. Then the total loss for all the $K$ candidates is $\mathcal{L}_{recon}=\sum_{k=1}^K\mathcal{L}_{recon}^k$.

% \paragraph{Distillation Loss.}
% We get the distilled pseudo label $\mathbf{d}\in\mathbb{R}^{M_\mathrm{p}}$ from the semantic matching module and the predict score $\mathbf{s}\in\mathbb{R}^{M_\mathrm{p}}$ from the predict module. The distillation loss is:
% \begin{equation}
% \mathcal{L}_{distill}=-\sum_{i=1}^{M_\mathrm{p}}d_i\operatorname{log}(s_i).
% \end{equation}

\paragraph{Multi-Task Loss}
We train the model end-to-end via a multi-task loss function, formulated by
\begin{equation}
\mathcal{L}_{overall}=\mathcal{L}_{distill}+\lambda_1\mathcal{L}_{cls}+\lambda_2\mathcal{L}_{match}+\lambda_3\mathcal{L}_{recon}
\end{equation}
where $\lambda_1$, $\lambda_2$ and $\lambda_3$ are hyper-parameters to balance four parts of the loss function.

\paragraph{Inference.}
Thanks to the knowledge distillation, all we need in the inference phase is the two-stage 3DVG pipeline. We get the predict score $\mathbf{s}\in\mathbb{R}^{M_\mathrm{p}}$ from the matching architecture, and the index of the predicted best-match proposal is $\operatorname{argmax}(\mathbf{s})$. Then, we obtain the corresponding 3D bounding box of this object proposal produced by the detector.

==> related/3dvg.tex <==
\noindent \textbf{Supervised 3D Visual Grounding.}
Grounding a sentence query in a 3D point cloud is a fundamental problem in vision-language tasks, with wide-ranging applications in fields like automatic robotics~\cite{xia2018gibson, wang2019reinforced, mittal2020attngrounder, feng2021cityflow} and AR/VR/metaverse~\cite{mystakidis2022metaverse, dionisio20133d}. The ScanRefer~\cite{chen2020scanrefer} and Referit3D~\cite{achlioptas2020referit3d} datasets annotate dense object-sentence correspondences on the widely-used 3D point cloud dataset Scannet~\cite{dai2017scannet}. By using the ground-truth object-sentence links, many advanced methods have been proposed for 3DVG.

Most recent 3D visual grounding methods~\cite{cai20223djcg, yuan2021instancerefer, zhao20213dvg, huang2022multi, huang2021text, yang2021sat} follow a two-stage pipeline. In the first stage, pre-trained 3D object detectors~\cite{qi2019deep, liu2021group} generate 3D object proposals. The second stage involves matching the selected object proposals with the sentence query. Existing two-stage methods improve performance by exploring the object attributes and relations between proposals in the second stage. For example, 3DVG-Transformer~\cite{zhao20213dvg} uses a coordinate-guided contextual aggregation module to capture relations between proposals and a multiplex attention module to distinguish the target object. TransRefer3D~\cite{he2021transrefer3d} uses an entity-aware attention module and a relation-aware attention module for fine-grained cross-modal matching. 3DJCG~\cite{cai20223djcg} devises a joint framework for 3D visual grounding~\cite{chen2020scanrefer} and 3D dense captioning~\cite{chen2021scan2cap} tasks, and their experiments demonstrate that extra caption-level data can improve the performance of 3D visual grounding.

In contrast to these supervised methods, our approach learns to localize target objects in 3D space using only caption-level annotations.

\noindent \textbf{Weakly Supervised Image Grounding. }
The image grounding task, similar to 3DVG, aims to identify objects in an image based on a sentence, and has a wide range of applications~\cite{plummer2015flickr30k, kazemzadeh2014referitgame, deng2021transvg, yu2018mattnet, kamath2021mdetr,yang2020improving}. Weakly supervised image grounding, which only requires images and corresponding sentences in the training phase, has gained popularity due to its elimination of expensive dense annotations~\cite{gupta2020contrastive, rohrbach2016grounding, wang2021improving, faghri2017vse++, datta2019align2ground}.

Weakly supervised image grounding is typically treated as a Multiple Instance Learning (MIL) problem~\cite{ilse2018attention,maron1997framework}, where the image is represented as a bag of regions, generated by a pre-trained image object detector. Image-sentence matching scores are calculated based on region-phrase similarity scores, and ground-truth image-sentence links are used to supervise these scores. For example, ARN~\cite{liu2019adaptive} pairs image proposals and queries based on subject, location, and context information through adaptive grounding and collaborative reconstruction. InfoGround~\cite{gupta2020contrastive} proposes a contrastive learning objective function~\cite{he2020momentum} to optimize image-sentence scores. Wang et al.~\cite{wang2021improving} use a pre-trained image object detector to generate pseudo category labels for all regions, achieving region-phrase alignment by distilling knowledge from these pseudo labels.

However, MIL-based weakly supervised image grounding methods cannot solve the weakly supervised problem in 3DVG. Firstly, the presence of numerous different objects in a single 3D scene makes it difficult to learn a stable MIL classifier. Secondly, while image grounding aims to locate objects corresponding to all phrases in the sentence, 3DVG requires the identification of a single target object, necessitating a deeper and more comprehensive understanding of the sentence's semantic information, rather than just its phrases.

% \noindent \textbf{Knowledge Distillation.} The technique of Knowledge Distillation\cite{hinton2015distilling} was developed for transferring knowledge from a teacher model to a student model. Recently, there has been a growing interest in using knowledge distillation for multi-modal learning\cite{luo2018graph,li2017large,gupta2016cross,garcia2018modality}, including applications in video captioning\cite{zhang2020object,pan2020spatio}, image captioning\cite{zhou2020more}, and image grounding\cite{wang2021improving}. In contrast to previous approaches, we propose to use a coarse-to-fine semantic matching model as the teacher model and a two-stage 3DVG model as the student model. We align the predicted referring scores of the 3DVG model with the distilled pseudo labels computed by the semantic matching model.

==> related/main.tex <==
\section{Related Work}
\label{sec:related_work}

\input{related/3dvg}

==> tables/reward.tex <==
\begin{table}[t]
\centering
% \tabcolsep=1mm
\caption{Ablation study on the matching score function.}
\label{table:reward}
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c|}{R@3, SUN} & \multicolumn{2}{c}{R@3, SCAN} \\ \cline{2-5} 
& & & & \\[-2ex]
                  & $m$=0.25         & $m$=0.5         & $m$=0.25        & $m$=0.5        \\ \midrule
One-hot           & 13.99            & 9.15            & 33.59           & 27.33          \\
Multi-hot         & 13.84            & 8.86            & 34.01           & 27.69          \\
Linear            & 14.05            & 9.31            & 34.03           & 27.25          \\
\textbf{Ours}     & \textbf{14.78}   & \textbf{9.55}   & \textbf{34.12}  & \textbf{27.97} \\ \bottomrule
\end{tabular}
\end{table}
